A Quantum Approximate Optimization Algorithm-based Decoder Architecture for NextG Wireless Channel Codes

Forward Error Correction (FEC) provides reliable data flow in wireless networks despite the presence of noise and interference. However, its processing demands significant fraction of a wireless network's resources, due to its computationally-expensive decoding process. This forces network designers to compromise between performance and implementation complexity. In this paper, we investigate a novel processing architecture for FEC decoding, one based on the quantum approximate optimization algorithm (QAOA), to evaluate the potential of this emerging quantum compute approach in resolving the decoding performance-complexity tradeoff. We present FDeQ, a QAOA-based FEC Decoder design targeting the popular NextG wireless Low Density Parity Check (LDPC) and Polar codes. To accelerate QAOA-based decoding towards practical utility, FDeQ exploits temporal similarity among the FEC decoding tasks. This similarity is enabled by the fixed structure of a particular FEC code, which is independent of any time-varying wireless channel noise, ambient interference, and even the payload data. We evaluate FDeQ at a variety of system parameter settings in both ideal (noiseless) and noisy QAOA simulations, and show that FDeQ achieves successful decoding with error performance at par with state-of-the-art classical decoders at low FEC code block lengths. Furthermore, we present a holistic resource estimation analysis, projecting quantitative targets for future quantum devices in terms of the required qubit count and gate duration, for the application of FDeQ in practical wireless networks, highlighting scenarios where FDeQ may outperform state-of-the-art classical FEC decoders.

==> related.tex <==
\section{Related Work}
\label{s: related}

The FEC decoding problem has been widely investigated from a classical computing perspective, where several decoding algorithms and their hardware implementation techniques have been developed \cite{hailes2015survey, 8616900}. Much focus has been dedicated towards designing approximate algorithms which sacrifice decoding performance but they enable efficient FPGA/ASIC hardware implementation. For LDPC codes, BP-based algorithms such as sum-product BP \cite{kschischang2001factor}, min-sum BP \cite{angarita2014reduced}, normalized and offset BP \cite{chen2002density} algorithms are widely employed for commercial applications and for Polar codes, SC-based algorithms such as SC List (list size $\leq$ 4) \cite{tal2015list}, SC Stack \cite{niu2012stack}, Stepped SC List \cite{rowshan2018stepped}, and simplified SC \cite{alamdar2011simplified} algorithms are most prevalent. These approximate algorithms all typically sacrifice 1--2 orders of bit error rate magnitude (specific values may be higher depending on the FEC code, wireless channel, and decoder parameters) in comparison to the Maximum-Likelihood decoding approach, thus limiting the net wireless communication throughput.

To address this problem and boost throughput, recent prior work has investigated quantum annealing (QA) based FEC decoding \cite{kasi2020towards, kasi2022design, bian2014discrete, chancellor2016direct}, which is substantially different from our proposed quantum-gate based \sysname{} decoding approach. Specifically, QA-based methods solve the FEC decoding problem via an adiabatic evolution of quantum state, where the input problem is specified to QA hardware using magnetic fields and magnetic couplings \cite{d2019technical}, whereas FDeQ solves the same problem by guiding the quantum state towards the solution using an alternating ansatz operator implemented using controllable quantum logic gates. \sysname{} provides several advantages over QA-based methods which we detail next.

Unlike \sysname{}, mapping problems to hardware is a significant challenge in QA-based approaches. This involves the use of additional ancillary qubits and finding a graph minor which itself is an NP-hard problem \cite{robertson1995graph}. To solve 8, 16, and 32 bit Polar decoding problems, QA-based approaches require 96, 352, and 1160 qubits respectively \cite{10246149}, whereas \sysname{} requires only 32, 80, and 192 qubits respectively for the same task. Similar advantage holds for LDPC codes as well. This is because sparse qubit connectivity demands additional qubits for resource routing in QA devices, whereas the same routing can be realized in FDeQ via SWAP operations that do not require additional qubits \cite{wille2014optimal}. It is also important to consider that unlike QA, quantum gate-based computing is a universal quantum computing approach pursued by wider industry consortia which we expect will help expedite the development of such devices and provide \sysname{} a more stable ground for FEC decoding.

Finally, we note that in current devices with high noise levels and imperfect qubits, both \sysname{} and QA-based approaches do not provide a speedup over classical methods \cite{kasi2020towards, kasi2022design}. Nevertheless, under ideal conditions, \sysname{} and QA are expected to provide exponential and quadratic speedups respectively over classical methods \cite{cerezo2021variational, villanueva2023adiabatic, roland2002quantum, vznidarivc2006exponential}. 




